Social Laws for Multi-agent Coordination in Stochastic Environments

In multi-agent environments, coordinating agents to prevent interference and ensure robust individual performance is a critical challenge. Previous research on social laws for multi-agent systems has primarily focused on deterministic, goal-based settings. This paper extends the concept of social laws to stochastic, reward-based environments, proposing a formalism for defining and verifying their robustness under various conditions. We introduce the notion of $\alpha$-robustness, a measure of the guaranteed utility each agent retains while pursuing its optimal single agent policy, assuming all agents obey the social law. We then present an approach for robustness verification of social laws in stochastic settings, based on a reduction to solving a series of Markov decision processes. Empirical evaluations on toy environments illustrate the potential of our framework.

==> mathprog.tex <==
\subsection{Basic Solution: Mathematical Programming}
We will look at stochastic policies and frame the robustness verification problems as a mathematical program.

% \subsection{Verifying Robustness}
Our decision variables will be the policy -- $\pi_i(s,a)$ (for every agent $i$, state $s$, and action $a$) denotes the probability that agent $i$ will pick action $a$ in state $s$.

The first two constraints ensures this is a valid policy:
\begin{equation}
\forall i,s: \sum_a \pi_i(s,a) = 1    
\end{equation}
and
\begin{equation}
\forall i,s,a: \pi_i(s,a) \geq 0
\end{equation}

We can also define helper variables for the value of state $s$ for agent $i$. These follow the Bellman equations, but here we define two versions:

The value for agent $i$ had it acted alone (that is, in its single agent projection), $V_{sap}^i(s)$ (for every agent $i$ and state $s$), is defined by:

\begin{multline}
\forall i, s: V_{sap}^i(s) = 
\sum_{a} \pi_i(s,a) \sum_{s'} P|_i(s,a,s') \\
\big(R^i(s,a,s') + \gamma V_{sap}^i(s')\big)
\end{multline}

Note that $P|_i(s,a,s')$ and $R^i(s,a,s')$ are constants, but $\pi_i(s,a)$ and $V_{sap}^i(s')$ are decision variables, and thus this constraint is bilinear.

On the other hand, the true value for agent $i$, when all agent actions are accounted for in the joint problem is:

\begin{multline}
\forall i, s: V_{joint}^i(s) = 
\sum_{a_1, \ldots, a_{|N|}} \prod_j \pi_j(s,a_j) \\
\sum_{s'} P(s,\langle a_1 \ldots, a_{|N|} \rangle ,s') \big(R^i(s,a,s') + \gamma V_{joint}^i(s')\big)
\end{multline}

Here, we multiply $|N|+1$ decision variables with each other -- the $|N|$ policy variables $\pi_j(s,a_j)$ and $V_{joint}^i(s')$. Thus, we have a non-linear optimization problem.


The above constraints define the dynamics of the system, and allow us to compute the value of the single agent projection and the value in the full system, for every agent and every combination of policies. However, to verify $\alpha$-robustness we must (i) ensure each agent follows a policy which is optimal in its single agent projection, and (ii) enforce (or falsify) that the joint value is worse than $\alpha$ times the value for the single agent projection.

% Finally, we add constraints for $\alpha$-robustness. 
First, we add constraints to ensure the policy is optimal assuming each agent acts alone. For ease of notation, we will assume we compute 
$\E_{s_0 \sim I} V^\ast_{\Pi_i}(s_0)$ beforehand, although this can be easily encoded into the same mathematical optimization problem using a separate set of decision variables for the policy.
Then we add the constraints:

\begin{equation}
\label{e:optimal}
\forall i: \sum_{s} I(s) V'_i(s) \geq 
\E_{s_0 \sim I} V^\ast_{\Pi_i}(s_0)
\end{equation}

Finally, we add the constraints which violate $\alpha$-robustness, by looking for a single agent which loses more than a factor of $\alpha$ in its utility:

\begin{equation}
\label{e:violate}
\exists i: \sum_{s} I(s) V_i(s) < \alpha \sum_{s} I(s) V'_i(s)
\end{equation}
(note that this can be encoded as a sum over the ReLU of the difference between the first term and the second term)

It is easy to see that if this mathematical optimization problem is feasible, then we have a set of stochastic policies $\pi_i \ldots \pi_{|N|}$, such that every agent $i$ can achieve its optimal utility by following $\pi_i$ alone (Eq. \ref{e:optimal}), but when all agents follow $\pi_i$, one of the agents loses more than a factor of $\alpha$ (Eq. \ref{e:violate}). Thus, the problem is feasible iff the MA setting is not $\alpha$-robust.

\subsection{Optimizing $\alpha$}

By making $\alpha$ a decision variable, and slightly modifying Eq. \ref{e:violate} to be 
\begin{equation}
\label{e:violate_opt}
\sum_i ReLU\big(\sum_{s} I(s) V_i(s) - \alpha \sum_{s} I(s) V'_i(s)\big) = 0
\end{equation}
we can now solve an optimization problem with the objective to maximize $\alpha$.
This will give us the maximal $\alpha$ for which the MA setting is robust (TODO: double check...)

\subsection{Encoding Social Laws}


% Note from Caleb: we should regularize how much the social law is restrictive

One simple way to encode a social law is to apply a minimum and a maximum over $\pi_i(s,a)$. We can encode this by adding two new types of decision variables: $l_i(s,a)$ and $u_i(s,a)$ which encode the lower and upper bound on the probability of agent $i$ choosing action $a$ in state $s$. We then add the constraints:

\begin{equation}
    \forall i, s, a: u_i(s,a) \geq \pi_i(s,a) \geq l_i(s,a)
\end{equation}

Adding this constraint allows our mathematical program to enact a social law, and we can then use the formulations for robustness verification or for optimizing $\alpha$ with either a fixed social law ($l, u$ are constants) or with the social law as a decision variable (in which case we optimize the social law).
